HMAE: Self-Supervised Few-Shot Learning for Quantum Spin Systems

Quantum machine learning for spin and molecular systems faces critical challenges of scarce labeled data and computationally expensive simulations. To address these limitations, we introduce Hamiltonian-Masked Autoencoding (HMAE), a novel self-supervised framework that pre-trains transformers on unlabeled quantum Hamiltonians, enabling efficient few-shot transfer learning. Unlike random masking approaches, HMAE employs a physics-informed strategy based on quantum information theory to selectively mask Hamiltonian terms based on their physical significance. Experiments on 12,500 quantum Hamiltonians (60% real-world, 40% synthetic) demonstrate that HMAE achieves 85.3% $\pm$ 1.5% accuracy in phase classification and 0.15 $\pm$ 0.02 eV MAE in ground state energy prediction with merely 10 labeled examples - a statistically significant improvement (p < 0.01) over classical graph neural networks (78.1% $\pm$ 2.1%) and quantum neural networks (76.8% $\pm$ 2.3%). Our method's primary advantage is exceptional sample efficiency - reducing required labeled examples by 3-5x compared to baseline methods - though we emphasize that ground truth values for fine-tuning and evaluation still require exact diagonalization or tensor networks. We explicitly acknowledge that our current approach is limited to small quantum systems (specifically limited to 12 qubits during training, with limited extension to 16-20 qubits in testing) and that, while promising within this regime, this size restriction prevents immediate application to larger systems of practical interest in materials science and quantum chemistry.

==> figures.tex <==
% LaTeX figures generated by the plot.py script
% You can input this file in your main LaTeX document using:
% \input{figures.tex}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/coeff_hist.png}
    \caption{Distribution of Hamiltonian coefficient magnitudes for representative quantum systems: (a) Heisenberg model, (b) transverse field Ising model, (c) molecular Hamiltonian, and (d) combined dataset. While individual model distributions show some deviations from Gaussian (especially discrete models), the aggregate distribution demonstrates reasonable approximation by a Gaussian mixture model (red curve).}
    \label{fig:coeff_hist}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/scaling_comparison.png}
    \caption{Performance retention vs. system size. The y-axis shows the performance normalized to 8-qubit performance (higher is better). HMAE (red) demonstrates superior retention of performance as system size increases, indicating better generalization to larger Hilbert spaces.}
    \label{fig:scaling_comparison}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/mutual_info.png}
    \caption{Information preservation across masking strategies. The y-axis shows prediction performance (higher indicates better information preservation) versus masking ratio (x-axis). Physics-informed masking (red) consistently preserves more task-relevant information than random masking and other approaches.}
    \label{fig:mutual_info}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/active_learning.png}
    \caption{Active learning performance curves. Left: Model performance vs. percentage of Hamiltonians simulated. Right: Computational resource usage vs. model performance. Active learning with HMAE (red) achieves significantly better resource efficiency than random sampling (blue).}
    \label{fig:active_learning}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/phase_discovery.png}
    \caption{Iterative phase discovery with active learning. From left to right: Phase boundaries after 10\%, 40\%, 70\%, and 100\% of the simulation budget. The active learning strategy progressively refines phase boundaries, focusing computational resources on the most uncertain regions.}
    \label{fig:phase_discovery}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/uncertainty_calibration.png}
    \caption{Uncertainty calibration for active learning. The plot shows predicted uncertainty (x-axis) versus observed error rate (y-axis). After calibration (red), the uncertainty estimates closely match the actual error rates, while uncalibrated estimates (blue) tend to be overconfident.}
    \label{fig:uncertainty_calibration}
\end{figure} \begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/coeff_hist.png}
    \caption{Coefficient histograms for different quantum Hamiltonian models.}
    \label{fig:coeff_hist}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/scaling_comparison.png}
    \caption{Performance retention versus system size for different quantum models.}
    \label{fig:scaling_comparison}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/mutual_info.png}
    \caption{Information preservation across different masking strategies.}
    \label{fig:mutual_info}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/active_learning.png}
    \caption{Performance and resource efficiency of active learning versus random sampling.}
    \label{fig:active_learning}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/phase_discovery.png}
    \caption{Phase diagram discovery at different simulation budget levels.}
    \label{fig:phase_discovery}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/uncertainty_calibration.png}
    \caption{Uncertainty calibration for active learning models.}
    \label{fig:uncertainty_calibration}
\end{figure}



==> figures/figures_code.tex <==
% LaTeX figures generated by the plot.py script
% You can use these figures in your main LaTeX document

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/qmi_verification.png}
    \caption{Empirical verification of our quantum information-theoretic approach: Comparison between theoretical predictions (solid lines) and measured QMI values (markers) across different masking strategies. Our optimal QMI-guided approach (red) consistently preserves more quantum information than alternatives.}
    \label{fig:qmi_verification}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/dimensional_consistency.png}
    \caption{Performance comparison of dimensionally consistent saliency with principled $\alpha_{opt}$ versus empirically tuned and suboptimal values across different system types. The principled approach (red) maintains optimal performance without hyperparameter tuning.}
    \label{fig:dimensional_consistency}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/entangled_phases_test.png}
    \caption{Performance on low-temperature entangled phases. The extended theoretical framework (red) maintains high performance across all quantum regimes, including highly entangled phases where the original framework (blue) shows significant degradation.}
    \label{fig:entangled_phases}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/masked_model_comparison.png}
    \caption{Performance comparison of masked-model approaches across system sizes. HMAE (our approach) maintains superior performance as system size increases, with the gap widening for larger systems.}
    \label{fig:masked_model_comparison}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/hierarchical_tokenization.png}
    \caption{Hierarchical tokenization scheme. (a) Standard binary representation with $O(n)$ scaling per token and $O(n^k)$ possible tokens. (b) Hierarchical representation with $O(\log n)$ scaling per token and $O((\log n)^k)$ possible tokens.}
    \label{fig:hierarchical_tokenization}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/memory_scaling.png}
    \caption{Memory requirements scaling with system size for standard vs. hierarchical tokenization. Y-axis is log-scale.}
    \label{fig:memory_scaling}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/absolute_scaling_perf.png}
    \caption{Absolute performance scaling with system size. Error bands represent 95% confidence intervals.}
    \label{fig:absolute_scaling_perf}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/cross_dataset_protocol.png}
    \caption{Cross-dataset evaluation protocol ensuring fair comparison across methods and datasets.}
    \label{fig:cross_dataset_protocol}
\end{figure}


